On the stability of the Brazilian presidential regime: a statistical analysis

Brazil's presidential system is characterized by the existence of many political parties that are elected for the Chamber of Deputies and unite in legislative coalitions to form a majority. Since the re-democratization in 1985, Brazil has had 8 direct presidential elections, among which there were two impeachments of the elected president. In this work we characterize the stability of the presidential regime and the periods of rupture analysing the votes that took place in the Chamber of Deputies from 1991 to 2019. We start by measuring the cohesion of the parties and the congress in the votes, quantifying the agreement between the votes of congressmen and observe that there is a stronger polarization among congressmen during legislative periods where there was no impeachment, referred to here as stable legislative periods. Using clustering algorithms, we are able to associate these polarized groups observed during the stable periods with the opposition to the government and government base. To characterize the impeachment of Dilma Roussef that happened in 2016 we analyze how the agreement between congressmen and the government evolved over time and identified, using cluster algorithms, that all the parties belonging to the majority coalition of the president, except her own party and another one, migrated to the opposition just before the impeachment. Our analyses allow us to identify some differences between stable presidential periods and Legislative terms with an impeachment.

==> dump.tex <==
Antiga tabela III que substituí pelo que fiz hoje dia 17/04

\begin{tabular}{c| l | l | l|c|l|l }
      Legis. & President                   & $G_1^2$ & $G_2^2$ & $G_1^2/\ndep$ &  ${\cal S}_1^2$ & ${\cal S}_2^2$ \\ \hline \hline 
      %     \multirow{2}{*}{49}      & Collor  &  356    & 151    &  0.7          &   \cb{0.8}     &  \cb{0.45}     \\
         \multirow           49  & Collor  &  356    & 151    &  0.7          &   \cb{0.8}     &  \cb{0.45}     \\
                                 & Itamar  &  400    & 106    &  0.79         &   \cb{0.8}     &  \cb{0.50}   \\\hline 
                             50  & FHC I   &  440    & 133    &  0.77         &   \cb{0.9}     &  \cb{0.30}   \\\hline 
                             51  & FHC II  &  402    & 161    &  0.71         &   \cb{0.9}     &  \cb{0.50}   \\\hline 
                             51  & Lula I  &  412    & 133    &  0.76         &   \cb{0.9}     &  \cb{0.50}   \\\hline 
                             53  & Lula II &  403    & 133    &  0.75         &   \cb{0.95}    &  \cb{0.40}    \\\hline 
                             54  & Dilma I &  438    & 115    &  0.79         &   \cb{0.85}    &  \cb{0.40}    \\\hline
     %    \multirow{2}{*}{55}     & Dilma II & 326    & 195    &  0.63         &   \cb{0.80}    &  \cb{0.40}   \\
         \multirow           55  & Dilma II & 326    & 195    &  0.63         &   \cb{0.80}    &  \cb{0.40}   \\            
                                 & Temer    & 414    & 120    &  0.78         &   \cb{xxx}     &  \cb{xxx}    \\\hline 
                             56  & Bolsonaro &\cb{xxx}  &\cb{xxx}  &\cb{xxx}  &    \cb{xxx}    &   \cb{xxx}     \\\hline 
\end{tabular}
